CLASS: Coronal Line Activity Spectroscopic Survey

We conduct the first systematic survey of a comprehensive set of the twenty optical coronal lines in the spectra of nearly 1 million galaxies observed by the Sloan Digital Sky Survey (SDSS) Data Release 8 catalog. This includes often overlooked high ionization-potential (IP) lines such as [Ar X] $\lambda$5533, [S XII] $\lambda$7609, [Fe XI] $\lambda$7892, and [Fe XIV] $\lambda$5303. We find that, given the limited sensitivity of SDSS, strong coronal line emission is extremely rare, with only $\sim 0.03$% of the sample showing at least one coronal line, significantly lower than the fraction of galaxies showing optical narrow line ratios ($\sim 17$%) or mid-infrared colors ($\sim 2$%) indicative of nuclear activity. The coronal line luminosities exhibit a large dynamic range, with values ranging from $\sim10^{34}$ to $10^{42}$ erg s$^{-1}$. We find that a vast majority ($\sim 80$%) of coronal line emitters in dwarf galaxies ($M_* < {9.6} \times 10^9$ M$_\odot$) do not display optical narrow line ratios indicative of nuclear activity, in contrast to higher mass galaxies ($\sim 17$%). Moreover, we find that the highest ionization potential lines are preferentially found in lower mass galaxies. These findings are consistent with the theory that lower mass black holes found in lower mass galaxies produce a hotter accretion disk, which in turn enhances the higher ionization coronal line spectrum. Future coronal line searches with 30 m class telescopes or JWST may provide a pathway into uncovering the intermediate mass black hole population.

==> Coronal Lines in SDSS Letter Revision arxiv/line_table_letter.tex <==

\startlongtable
\begin{deluxetable*}{lccccccc}
\tabletypesize{\footnotesize}
\tablecaption{Optical coronal emission lines from 3346--7892 \AA. For the luminosity, the values shown are (mean) $\pm$ (standard deviation). The detection confidence levels are 68\%.}
\tablehead{\colhead{Line} & \colhead{Wavelength}\textsuperscript{1} & \colhead{Critical Density} & \colhead{Ionization Potential}\textsuperscript{2} & \colhead{Transition} &\colhead{Luminosity} & \colhead{Detections} & \colhead{Number} \\
\colhead{} & \colhead{(\AA)} & \colhead{(cm$^{-3}$)} & \colhead{(eV)} & \colhead{} & \colhead{$\log L/$erg s$^{-1}$ (dex)} & \colhead{(\%)} & \colhead{}}
\decimals
\startdata
\lbrack \ion{Fe}{11}\rbrack & 7891.800 & $6.39 \times 10^8$ & 262.10 & $^3$P$_2 - ^3$P$_1$ & $38.92 \pm 1.27$ & ${0.0064}^{+0.0029}_{-0.0021}$ & 9 \\ 
\lbrack \ion{S}{12}\rbrack & 7611.000 & $7.09 \times 10^9$ & 504.78 & $^2$P$^0_{1/2} - ^2$P$^0_{3/2}$ & $39.40 \pm 0.28$ & ${0.00058}^{+0.00076}_{-0.00037}$ & 2 \\ 
\lbrack \ion{Fe}{10}\rbrack & 6374.510 & $4.45 \times 10^8$ & 235.04 & $^2$P$^0_{3/2} - ^2$P$^0_{1/2}$ & $39.00 \pm 1.05$ & ${0.0407}^{+0.0043}_{-0.0039}$ & 107 \\ 
\lbrack \ion{Fe}{7}\rbrack & 6087.000 & $4.46 \times 10^7$ & 99.00 & $^3$F$_3 - ^1$D$_2$ & $39.96 \pm 0.59$ & ${0.0146}^{+0.0015}_{-0.0014}$ & 111 \\ 
\lbrack \ion{Fe}{7}\rbrack & 5720.700 & $3.72 \times 10^7$ & 99.00 & $^3$F$_2 - ^1$D$_2$ & $39.77 \pm 0.59$ & ${0.0158}^{+0.0016}_{-0.0015}$ & 114 \\ 
\lbrack \ion{Ar}{10}\rbrack & 5533.265 & $2.36 \times 10^9$ & 422.60 & $^2$P$^0_{3/2} - ^2$P$^0_{1/2}$ & $38.83 \pm 2.83$ & ${0.0028}^{+0.0019}_{-0.0012}$ & 5 \\ 
\lbrack \ion{Fe}{6}\rbrack & 5335.180 & $6.32 \times 10^6$ & 75.00 & $^4$F$_{3/2} - ^4$P$_{1/2}$ & $39.74 \pm 2.14$ & ${0.00131}^{+0.00064}_{-0.00045}$ & 8 \\ 
\lbrack \ion{Ca}{5}\rbrack & 5309.110 & $6.63 \times 10^7$ & 67.10 & $^3$P$_2 - ^1$D$_2$ & $40.11 \pm 0.58$ & ${0.00137}^{+0.00055}_{-0.00040}$ & 11 \\ 
\lbrack \ion{Fe}{14}\rbrack & 5302.860 & $3.99 \times 10^8$ & 361.00 & $^2$P$^0_{1/2} - ^2$P$^0_{3/2}$ & $39.94 \pm 0.66$ & ${0.00095}^{+0.00051}_{-0.00035}$ & 7 \\ 
\lbrack \ion{Fe}{7}\rbrack & 5276.380 & $2.98 \times 10^6$ & 99.00 & $^3$F$_4 - ^3$P$_2$ & $37.08 \pm 1.76$ & ${0.0057}^{+0.0026}_{-0.0018}$ & 9 \\ 
\lbrack \ion{Fe}{6}\rbrack & 5176.040 & $3.29 \times 10^7$ & 75.00 & $^4$F$_{9/2} - ^2$G$_{9/2}$ & $39.47 \pm 2.55$ & ${0.00070}^{+0.00068}_{-0.00038}$ & 3 \\ 
\lbrack \ion{Fe}{7}\rbrack & 5158.890 & $3.44 \times 10^6$ & 99.00 & $^3$F$_3 - ^3$P$_1$ & $37.70 \pm 1.45$ & ${0.0025}^{+0.0020}_{-0.0012}$ & 4 \\ 
\lbrack \ion{Fe}{6}\rbrack & 5145.750 & $2.29 \times 10^7$ & 75.00 & $^4$F$_{7/2} - ^2$G$_{7/2}$ & $40.65 \pm 0.48$ & ${0.00077}^{+0.00041}_{-0.00028}$ & 7 \\ 
\lbrack \ion{Fe}{7}\rbrack & 4893.370 & $3.09 \times 10^6$ & 99.00 & $^3$F$_2 - ^3$P$_1$ & $38.94 \pm 2.21$ & ${0.0054}^{+0.0036}_{-0.0023}$ & 5 \\ 
\lbrack \ion{Fe}{5}\rbrack & 4180.600 & $1.86 \times 10^8$ & 54.80 & $^5$D$_1 - ^3$P2$_0$ & $39.45 \pm 2.15$ & ${0.00117}^{+0.00079}_{-0.00051}$ & 5 \\ 
\lbrack \ion{Fe}{5}\rbrack & 3891.280 & $1.61 \times 10^8$ & 54.80 & $^5$D$_4 - ^3$F2$_4$ & $40.62 \pm 1.06$ & ${0.00022}^{+0.00029}_{-0.00014}$ & 2 \\ 
\lbrack \ion{Fe}{5}\rbrack & 3839.270 & $1.00 \times 10^8$ & 54.80 & $^5$D$_3 - ^3$F2$_3$ & $41.20 \pm 0.60$ & ${0.00054}^{+0.00037}_{-0.00023}$ & 5 \\ 
\lbrack \ion{Fe}{7}\rbrack & 3758.920 & $4.02 \times 10^7$ & 99.00 & $^3$F$_4 - ^1$G$_4$ & $40.38 \pm 0.90$ & ${0.00097}^{+0.00048}_{-0.00033}$ & 8 \\ 
\lbrack \ion{Ne}{5}\rbrack & 3425.881 & $1.90 \times 10^7$ & 97.11 & $^3$P$_2 - ^1$D$_2$ & $41.21 \pm 0.29$ & ${0.0123}^{+0.0018}_{-0.0016}$ & 61 \\ 
\lbrack \ion{Ne}{5}\rbrack & 3345.821 & $1.14 \times 10^7$ & 97.11 & $^3$P$_1 - ^1$D$_2$ & $40.91 \pm 0.24$ & ${0.0085}^{+0.0018}_{-0.0015}$ & 31 \\ 
\enddata
\begin{tablenotes}
    \item[1] \textsuperscript{1}Wavelengths taken from: \url{https://physics.nist.gov/PhysRefData/ASD/lines_form.html}.
    \item[2] \textsuperscript{2}Ionization potential taken from: \url{https://physics.nist.gov/PhysRefData/ASD/ionEnergy.html}.
\end{tablenotes}
\label{tab:lines}
\end{deluxetable*}

